Compact Tetrahedralization-based Acceleration Structure for Ray Tracing

We propose a compact and efficient tetrahedral mesh representation to improve the ray-tracing performance. We reorder tetrahedral mesh data using a space-filling curve to improve cache locality. Most importantly, we propose an efficient ray traversal algorithm. We provide details of common ray tracing operations on tetrahedral meshes and give the GPU implementation of our traversal method. We demonstrate our findings through a set of comprehensive experiments. Our method outperforms existing tetrahedral mesh-based traversal methods and yields comparable results to the traversal methods based on the state of the art acceleration structures such as k-dimensional (k-d) trees and Bounding Volume Hierarchies (BVHs).

==> build_and_render_times/table.tex <==
\begin{table*}[htbp]
\centering
\small
\caption{The computational costs of acceleration structures and rendering times for traversal methods}
\begin{tabular}{|lrrrrr|}
\hline
\multicolumn{6}{|c|}{Scenes}\\
\hline
& \multicolumn{1}{c}{Torus Knots}
& \multicolumn{1}{c}{Torus Knots in a Box}
& \multicolumn{1}{c}{Armadillo}
& \multicolumn{1}{c}{Armadillo in a Box}
& \multicolumn{1}{c|}{Neptune}
\\
& \includegraphics[width = 0.14\textwidth]{{"build_and_render_times/Torus Knots"}.png} & \includegraphics[width = 0.14\textwidth]{{"build_and_render_times/Torus Knots in a Box"}.png} & \includegraphics[width = 0.14\textwidth]{{"build_and_render_times/Armadillo"}.png} & \includegraphics[width = 0.14\textwidth]{{"build_and_render_times/Armadillo in a Box"}.png} & \includegraphics[width = 0.14\textwidth]{{"build_and_render_times/Neptune"}.png} \\
\hline
%\multicolumn{6}{}{}\\
\hline
\multicolumn{6}{|c|}{Scene statistics} \\
\hline
\# of triangles & 77,760 & 77,772 & 345,938 & 345,950 & 448,896 \\
\hline
%\multicolumn{6}{}{}\\
\hline
\multicolumn{6}{|c|}{Construction times (in seconds)} \\
\hline
Tet-mesh-ScTP~\cite{Lagae:2008:Constrained}& 3.596 & 3.638 & 16.733 & 20.252 & 79.822 \\
Tet-mesh-80~\cite{Maria:2017:Traversal}& 3.656 & 3.663 & 16.595 & 20.143 & 79.657 \\
Tet-mesh-32& 3.753 & 3.643 & 16.659 & 20.262 & 79.536 \\
Tet-mesh-20& 3.778 & 3.658 & 16.704 & 20.444 & 79.573 \\
Tet-mesh-16& 3.640 & 3.524 & 16.546 & 19.919 & 79.846 \\
BVH~\cite{Matt:2016:Pbr}& \textbf{0.078} & \textbf{0.079} & \textbf{0.391} & \textbf{0.396} & \textbf{0.474} \\
\textit{k}-d tree~\cite{Matt:2016:Pbr}& 0.739 & 0.590 & 1.454 & 1.651 & 2.265 \\
\hline
%\multicolumn{6}{}{}\\
\hline
\multicolumn{6}{|c|}{Rendering times (in milliseconds)} \\
\hline
Tet-mesh-ScTP~\cite{Lagae:2008:Constrained}& 261.5 & 293.4 & 232.5 & 306.7 & 268.9 \\
Tet-mesh-80~\cite{Maria:2017:Traversal}& 244.1 & 278.9 & 218.1 & 262.4 & 236.5 \\
Tet-mesh-32& 150.7 & 181.7 & 148.5 & 182.5 & 158.7 \\
Tet-mesh-20& \textbf{125.8} & \textbf{142.3} & 117.1 & 145.3 & 127.1 \\
Tet-mesh-16& 136.3 & 152.4 & 124.6 & 153.2 & 135.9 \\
BVH~\cite{Matt:2016:Pbr}& 152.7 & 192.2 & \textbf{78.1} & \textbf{126.1} & \textbf{78.7} \\
\textit{k}-d tree~\cite{Matt:2016:Pbr}& 139.9 & 214.4 & 85.7 & 182.3 & 81.7 \\
\hline
%\multicolumn{6}{}{}\\
\hline
\multicolumn{6}{|c|}{Scenes}\\
\hline
& \multicolumn{1}{c}{Neptune in a Box}
& \multicolumn{1}{c}{Mix}
& \multicolumn{1}{c}{Mix in a Box}
& \multicolumn{1}{c}{Mix close}
& \multicolumn{1}{c|}{Mix in a Box close}
\\
& \includegraphics[width = 0.14\textwidth]{{"build_and_render_times/Neptune in a Box"}.png} & \includegraphics[width = 0.14\textwidth]{{"build_and_render_times/Mix"}.png} & \includegraphics[width = 0.14\textwidth]{{"build_and_render_times/Mix in a Box"}.png} & \includegraphics[width = 0.14\textwidth]{{"build_and_render_times/Mix close"}.png} & \includegraphics[width = 0.14\textwidth]{{"build_and_render_times/Mix in a Box close"}.png} \\
\hline
%\multicolumn{6}{}{}\\
\hline
\multicolumn{6}{|c|}{Scene statistics} \\
\hline
\# of triangles & 448,908 & 2,505,992 & 2,506,004 & 2,505,992 & 2,506,004 \\
\hline
%\multicolumn{6}{}{}\\
\hline
\multicolumn{6}{|c|}{Construction times (in seconds)} \\
\hline
Tet-mesh-ScTP~\cite{Lagae:2008:Constrained}& 155.478 & 124.208 & 170.216 & 124.840 & 485.950 \\
Tet-mesh-80~\cite{Maria:2017:Traversal}& 156.381 & 125.081 & 169.116 & 125.068 & 482.908 \\
Tet-mesh-32& 153.788 & 124.000 & 169.502 & 123.183 & 487.291 \\
Tet-mesh-20& 155.580 & 124.087 & 169.890 & 124.015 & 483.827 \\
Tet-mesh-16& 154.644 & 124.493 & 170.175 & 123.401 & 484.516 \\
BVH~\cite{Matt:2016:Pbr}& \textbf{0.487} & \textbf{2.968} & \textbf{3.017} & \textbf{2.966} & \textbf{2.997} \\
\textit{k}-d tree~\cite{Matt:2016:Pbr}& 2.471 & 13.889 & 14.668 & 13.846 & 16.624 \\
\hline
%\multicolumn{6}{}{}\\
\hline
\multicolumn{6}{|c|}{Rendering times (in milliseconds)} \\
\hline
Tet-mesh-ScTP~\cite{Lagae:2008:Constrained}& 279.6 & 402.6 & 430.0 & 449.5 & 455.0 \\
Tet-mesh-80~\cite{Maria:2017:Traversal}& 261.0 & 355.7 & 384.7 & 411.2 & 419.6 \\
Tet-mesh-32& 176.1 & 247.2 & 268.5 & 265.5 & 269.9 \\
Tet-mesh-20& 137.0 & 196.3 & 211.1 & 205.6 & \textbf{210.2} \\
Tet-mesh-16& 152.0 & 223.9 & 241.4 & 237.4 & 240.3 \\
BVH~\cite{Matt:2016:Pbr}& \textbf{120.4} & 144.6 & \textbf{187.9} & 224.9 & 253.8 \\
\textit{k}-d tree~\cite{Matt:2016:Pbr}& 162.6 & \textbf{143.5} & 214.8 & \textbf{193.1} & 213.6 \\
\hline
%\multicolumn{6}{}{}\\
%\hline
\end{tabular}
\label{tab:build_and_render_times}
\end{table*}

\begin{table*}[htbp]
\centering
\caption{\color{red}{The computational costs of acceleration structures and rendering times for traversal methods (remeshed scenes).}}
\begin{tabular}{|lrrrrr|}
\hline
\multicolumn{6}{|c|}{Scenes}\\
\hline
& \multicolumn{1}{c}{Rungholt Far}
& \multicolumn{1}{c}{Rungholt Default}
& \multicolumn{1}{c}{Rungholt Close}
& \multicolumn{1}{c}{Exhaust Pipe Left}
& \multicolumn{1}{c|}{Exhaust Pipe Right}
\\
& \includegraphics[width = 0.14\textwidth]{{"build_and_render_times/Rungholt Far"}.png} & \includegraphics[width = 0.14\textwidth]{{"build_and_render_times/Rungholt Default"}.png} & \includegraphics[width = 0.14\textwidth]{{"build_and_render_times/Rungholt Close"}.png} & \includegraphics[width = 0.14\textwidth]{{"build_and_render_times/Exhaust Pipe Left"}.png} & \includegraphics[width = 0.14\textwidth]{{"build_and_render_times/Exhaust Pipe Right"}.png} \\
\hline
%\multicolumn{6}{}{}\\
\hline
\multicolumn{6}{|c|}{Scene statistics} \\
\hline
\# of triangles & 3,580,928 & 3,580,928 & 3,580,928 & 6,244,678 & 6,244,678 \\
\hline
%\multicolumn{6}{}{}\\
\hline
\multicolumn{6}{|c|}{Construction times (in seconds)} \\
\hline
BVH~\cite{Matt:2016:Pbr}& 4.230 & 4.247 & 4.212 & 7.771 & 7.767 \\
\textit{k}-d tree~\cite{Matt:2016:Pbr}& 37.140 & 37.078 & 37.039 & 66.462 & 66.403 \\
\hline
%\multicolumn{6}{}{}\\
\hline
\multicolumn{6}{|c|}{Rendering times (in milliseconds)} \\
\hline
Tet-mesh-ScTP~\cite{Lagae:2008:Constrained}& 554.035 & 525.523 & 436.716 & 333.291 & 344.483 \\
Tet-mesh-80~\cite{Maria:2017:Traversal}& 488.299 & 466.933 & 400.589 & 312.152 & 320.361 \\
Tet-mesh-32& 353.444 & 333.274 & 265.337 & 202.472 & 207.239 \\
Tet-mesh-20& 282.211 & 265.337 & 215.118 & 163.814 & 166.619 \\
Tet-mesh-16& 313.335 & 293.351 & 238.027 & 183.198 & 186.125 \\
BVH~\cite{Matt:2016:Pbr}& 198.140 & 227.333 & 243.165 & 177.263 & 187.540 \\
\textit{k}-d tree~\cite{Matt:2016:Pbr}& \textbf{119.589} & \textbf{127.948} & \textbf{126.434} & \textbf{114.358} & \textbf{121.114} \\
\hline
\multicolumn{6}{}{}\\
\end{tabular}
\label{tab:build_and_render_times_remesh}
\end{table*}


==> memory_usage/table.tex <==
\begin{table*}[b]
\centering
\small
\caption{\color{red}{The memory requirements of tetrahedral mesh-based acceleration structures}}
\begin{tabular}{|lrrrrrr|}
\hline
\multicolumn{7}{|c|}{Scenes}\\
\hline
& \multicolumn{1}{c}{Torus Knots}
& \multicolumn{1}{c}{Armadillo}
& \multicolumn{1}{c}{Neptune}
& \multicolumn{1}{c}{Mix}
& \multicolumn{1}{c}{Rungholt}
& \multicolumn{1}{c|}{Exhaust Pipe}
\\
& \includegraphics[width = 0.12\textwidth]{{"memory_usage/Torus Knots"}.png} & \includegraphics[width = 0.12\textwidth]{{"memory_usage/Armadillo"}.png} & \includegraphics[width = 0.12\textwidth]{{"memory_usage/Neptune"}.png} & \includegraphics[width = 0.12\textwidth]{{"memory_usage/Mix"}.png} &
\includegraphics[width = 0.12\textwidth]{{"memory_usage/Rungholt Default"}.png} &
\includegraphics[width = 0.12\textwidth]{{"memory_usage/Exhaust Pipe Left"}.png} \\
\hline
%\multicolumn{7}{}{}\\
\hline
\multicolumn{7}{|c|}{Scene statistics} \\
\hline
\# of triangles & 77,760 & 345,938 & 448,896 & 2,505,992 & 3,580,928 & 6,244,678\\
\hline
%\multicolumn{7}{}{}\\
\hline
\multicolumn{7}{|c|}{Accelerator size (in megabytes)} \\
\hline
Tet-mesh-32& 12.3 & 49.4 & 61.2 & 352.1 & 406.1 & 885.1 \\
Tet-mesh-20& 9.2 & 37.7 & 47.0 & 269.0 & 310.2 & 673.6 \\
Tet-mesh-16& \textbf{8.2} & \textbf{33.7} & \textbf{42.2} & \textbf{241.3} & \textbf{278.2} & \textbf{603.1} \\
Tet-mesh-80~\cite{Maria:2017:Traversal}& 20.6 & 78.4 & 94.6 & 553.8 & 639.4 & 1410.0 \\
\hline
\end{tabular}
\label{tab:memory_usage}
\end{table*}


==> render_times_gpu/table.tex <==
\begin{table*}[htbp]
\centering
\caption{\color{red}{The Rendering times of tetrahedral mesh-based acceleration structures on the GPU}}
\begin{tabular}{|lrrrrrr|}
\hline
\multicolumn{7}{|c|}{Scenes}\\
\hline
& \multicolumn{1}{c}{Torus Knots}
& \multicolumn{1}{c}{Armadillo}
& \multicolumn{1}{c}{Neptune}
& \multicolumn{1}{c}{Mix}
& \multicolumn{1}{c}{Rungholt}
& \multicolumn{1}{c|}{Exhaust Pipe}
\\
& \includegraphics[width = 0.115\textwidth]{{"memory_usage/Torus Knots"}.png} & \includegraphics[width = 0.115\textwidth]{{"memory_usage/Armadillo"}.png} & \includegraphics[width = 0.115\textwidth]{{"memory_usage/Neptune"}.png} & \includegraphics[width = 0.115\textwidth]{{"memory_usage/Mix"}.png} &
\includegraphics[width = 0.115\textwidth]{{"memory_usage/Rungholt Default"}.png} &
\includegraphics[width = 0.12\textwidth]{{"memory_usage/Exhaust Pipe Left"}.png} \\
\hline
%\multicolumn{7}{}{}\\
\hline
\multicolumn{7}{|c|}{Scene statistics} \\
\hline
\# of triangles & 77,760 & 345,938 & 448,896 & 2,505,992 & 3,580,928 & 6,244,678 \\
\hline
%\multicolumn{7}{}{}\\
\hline
\multicolumn{7}{|c|}{Kernel execution time (in milliseconds)} \\
\hline
Tet-mesh-ScTP~\cite{Lagae:2008:Constrained}& 20.021	& 19.612 & 20.898 & 43.910 &		43.633 & 22.560 \\
Tet-mesh-80~\cite{Maria:2017:Traversal}& 7.790 & 7.136 & 7.941 & 13.454 & 14.360 & 9.023 \\
Tet-mesh-32& 19.541	& 18.950 & 20.958 & 42.690 & 44.544 & 21.320 \\
Tet-mesh-20& \textbf{6.156} & \textbf{5.803} & \textbf{6.529} & \textbf{11.322} & \textbf{12.172} & \textbf{6.931} \\
Tet-mesh-16& 7.120 & 6.477 & 7.328 & 12.157 & 13.444 & 8.231 \\

\hline
\end{tabular}
\label{tab:render_times_gpu}
\end{table*}

